Collapse or Thrive? Perils and Promises of Synthetic Data in a Self-Generating World

What happens when generative machine learning models are pretrained on web-scale datasets containing data generated by earlier models? Some prior work warns of "model collapse" as the web is overwhelmed by synthetic data; other work suggests the problem can be contained (i.e. collapse can be avoided) by managing how available data are used in pretraining. In this paper, we report experiments on three ways of using data (training-workflows), across three generative model task-settings (multivariate Gaussian estimation, kernel density estimation, and language-model fine-tuning) to further confirm the possibility of containment: (a) we confirm that the training-workflow of {\it replacing} all real data by successive generations of purely synthetic data indeed suffers model collapse in all task-settings studied; (b) we consider the training-workflow of {\it accumulating} synthetic data alongside real data and training on all data combined and confirming that, although the proportion of real data eventually becomes zero, models remain stable and their test losses do not diverge under this training-workflow; (c) we consider a training-workflow where real and synthetic data accumulate together but successive generations of pretraining are constrained to use fixed-size data subsets each generation. In this workflow, we observe slow and gradual rather than explosive degradation of test loss performance across generations. Our insights are particularly important when forecasting whether future frontier generative models will collapse or thrive, and our results open avenues for empirically and mathematically studying the context-dependent value of synthetic data.

==> 02_related_work.tex <==
\section{Related Work}

The limitations of using AI-generated images to train other image models have been well-documented since 2022 \citep{hataya2023will}. 
\citet{shumailov2023curse} initially sounded the alarm about synthetic data for training language models by showing that a model trained repeatedly on its own outputs exhibits severely denigrated quality. Shumailov's theory and empirical work were quickly extended to many new settings (\cite{alemohammad2023self, bertrand2023stability, dohmatob2024tale, dohmatob2024model, marchi2024heatdeathgenerativemodels}).  

% While most of the theory concerning model collapse is limited to specific statistical models, recently \cite{marchi2024heatdeathgenerativemodels} has provided theoretical conditions under which deep generative models collapse. 

Within the model collapse literature, a variety of data dynamics have been studied, which vary in how ``real'' data is discarded or retained, how ``synthetic'' data is generated, and how each is (or is not) incorporated into future training sets (\cite{martinez2023combining,mobahi2020self,dohmatob2024model}). A common feature of many of these is that at least some real data is discarded, often because total dataset size is kept constant across model-fitting iterations. However, \cite{gerstgrasser2024modelcollapseinevitablebreaking} note that this may not represent real-world dynamics, and that model collapse is avoided when data accumulates. What is not clear, however, is whether this claim holds universally, including in the specific settings studied in other prior work. We help close this gap by extending Gerstgrasser's empirical and theoretical analyses to several of these settings.  
 
Where model collapse can be seen as studying a worst-case scenario, it has also been observed that \textit{some} kinds of synthetic data have a positive effect.  \cite{dohmatob2024tale} and \cite{jain2024scalinglawslearningreal} find that certain amounts of synthetic data can improve model performance, and \cite{ferbach2024selfconsuminggenerativemodelscurated} suggest that with curation, self-consuming loops can improve alignment with human preferences. A growing literature on how to filter and harness synthetic data has achieved impressive results on a variety of benchmarks (\cite{STaR, li2024mugglemathassessingimpactquery, yang2024syntheticcontinuedpretraining}), raising interesting questions about the limits of when unfiltered synthetic data can help. 
 In this vein, we answer a question posed by \cite{gerstgrasser2024modelcollapseinevitablebreaking}: does the proportion or the raw amount of real data in a mixed training set have a greater impact on test loss?  In the process, we find that proportionally small amounts of synthetic data can improve test loss when real data is scarce.
